Efficient Iterative Programs with Distributed Data Collections

Big data programming frameworks have become increasingly important for the development of applications for which performance and scalability are critical. In those complex frameworks, optimizing code by hand is hard and time-consuming, making automated optimization particularly necessary. In order to automate optimization, a prerequisite is to find suitable abstractions to represent programs; for instance, algebras based on monads or monoids to represent distributed data collections. Currently, however, such algebras do not represent recursive programs in a way which allows for analyzing or rewriting them. In this paper, we extend a monoid algebra with a fixpoint operator for representing recursion as a first class citizen and show how it enables new optimizations. Experiments with the Spark platform illustrate performance gains brought by these systematic optimizations.

==> proof.tex <==

\subsection{Condition for pushing a filter}\label{app:pushfilt}
\subsubsection{More properties of fixpoint expressions} \label{app:morefixprop}

We have:

$\fixptn{R}{\varphi} = \bigcup_{n \in \N} \varphi^{(n)}(R) = \bigcup_{n \in \N} \varphi{(\biguplus_{r \in R}\singleton{r})} = \bigcup_{n \in \N} (\biguplus_{r \in R}\varphi(\singleton{r})) = \bigcup_{n \in \N} (\bigcup_{r \in R}\varphi(\singleton{r}))$.

Which means that $\forall a \in \fixptn{R}{\varphi} \;\;\; a \in \varphi^{(n)}(\singleton{r})$ for some $r \in R$ and $n \in N$.

Also, $a \in \distinct{\varphi^{(n)}(\singleton{r})}$ and $\forall n \in \N \; \forall r\in R \;\;\; \distinct{\varphi^{(n)}(\singleton{r})} \subset \fixptn{R}{\varphi}$. 

\subsubsection{Proof for Sec.~\ref{sec:filter}}
Let $A = \flatmap{\pi}{\ite{c(a)}{\singleton{\pi}}{\singleton{}}}{\fixptn{R}{\varphi}}$

And let the condition (C) be:
$\forall r \in R  \quad \forall s \in \varphi(\singleton{r}) \quad \pi_a(r) = \pi_a(s)$

We note $(*)$ the following proposition: $\forall s\in \fixptn{R}{ \varphi} \quad \exists r \in R \quad \pi_a(r) = \pi_a(s)$ 

$(*)$ is verified when the condition (C) is fulfilled because $$\forall s\in \fixptn{R}{\varphi} \quad \exists r \in R \quad \exists n \in \N \quad s\in \varphi^{(n)}(\singleton{r}) \text{ (shown in Appendix~\ref{app:morefixprop})}$$.
We show that $A = \fixptn{F(R)}{\varphi}$  when the condition (C) is fulfilled:
\begin{enumerate}

\item $\fixptn{F(R)}{\varphi} \subset A$:

$F(R) \subset R \implies \fixptn{F(R)}{\varphi} \subset \fixptn{R}{\varphi} \quad$ (because $\fixptn{R}{\varphi} = \fixptn{F(R) \bunion R'}{\varphi} = \fixptn{F(R)}{\varphi} \sunion \fixptn{R'}{\varphi}$ and \fixptn{R}{\varphi} does not contain duplicates)

Let $s \in \fixptn{F(R)}{\varphi}$

$\exists r \in F(R) \quad \pi_a(s) = \pi_a(r)  \quad (*)$

So $c(\pi_a(s)) = c(\pi_a(r))=\text{true \quad (because } r\in F(R))$

So $s\in \fixptn{R}{\varphi}$ and $c(\pi_a(s))$ is true, then $s\in A$


\item $A \subset \fixptn{F(R)}{\varphi} $: 

Let $s\in A. \text{ We have:} \quad s \in \fixptn{R}{\varphi} \text{ and } c(\pi_a(s)) = \text{true}$ 

So $\exists r \in R \quad \exists n \in \N \quad \pi_a(s) = \pi_a(r) \quad (\text{because } (*) \text{ and } s \in \varphi^{(n)}(\singleton{r}))$

So $c(\pi_a(r)) = c(\pi_a(s)) = \text{true}$ 

So $r \in F(R)$, which means $\distinct{\varphi^{(n)}(\singleton{r})} \subset \fixptn{F(R)}{\varphi}$ (see fixpoint related proofs in Appendix~\ref{app:morefixprop}), so $s \in \fixptn{F(R)}{\varphi}$.

\end{enumerate}

\subsection{$\fixpointdistRule$ proof}\label{app:distloop}
Let us suppose there exist a pattern variable $a$ for which $(C_a)$ is verified, and let us suppose $(P_a)$.
Let $R_i$ and $R_j$ partitions of $R$ such that $i \neq j$.
We have $\forall s\in \fixptn{R}{ \varphi} \quad \exists r \in R \quad \pi_a(r) = \pi_a(s)$ because $(C_a)$ as mentioned in Appendix~\ref{app:pushfilt}.
Which means that for any $x \in \fixptn{R_i}{\varphi}$ and $y \in \fixptn{R_j}{\varphi}$, $\exists r_i \in R_i \; \exists r_j \in R_j \;\;\; \pi_a(r_i) = \pi_a(x) \text{ and } \pi_a(r_j) = \pi_a(y)$. We have $\pi_a(r_i) \neq \pi_a(r_j)$ because $(P_a)$, so $x \neq y$. Hence $\forall i \neq j \;\; \fixptn{R_i}{\varphi} \cap \fixptn{R_j}{\varphi} = \emptyset$.

\subsection{\semijoinRule{} proofs}\label{app:pushsemijoin}
\packedsubsubsection{Inserting $\semijoinfilter{}$ before the join}\label{app:pushsemijoin1}

We have $join(A,B) = \setcomp{(k,(x,y))}{(k,x) \in A, (k,y) \in B}$.

So $(k,(x,y)) \in join(A,B) \iff (k,x) \in A \land (k,y) \in B \iff (k,x) \in A \land ((k,y) \in B \land \exists w \; (k,w)~\in~A) \iff (k,x) \in A \;\land\; (k,y) \in \semijoinfilter{B} \iff (k,(x,y)) \in join(A,\semijoinfilter{B}))$.


\packedsubsubsection{$\semijoinfilter{}$ is a filter}\label{app:pushsemijoin2}
We can show that
$\semijoinfilter{B} = \flatmap{(k,v)}{\ite{c(k)}{\singleton{(k,v)}}{\singleton{}}}{B}$

where $c(k)$ is the boolean expression that corresponds to the predicate $\exists w (k,w) \in A$.

This expression can be: $c(k) = \reduce{\vee}{\flatmap{(k',a)}{k==k'}{A}}$.

Which means that in case $\varphi$ fulfills the criteria for pushing filters we will have $\semijoinfilter{B} = \semijoinfilter{\fixptn{R}{\varphi}} = \fixptn{\semijoinfilter{R}}{\varphi}$.



\packedsubsubsection{Rewriting the filter with a cogroup}\label{app:pushsemijoin3}

We show that $\semijoinfilter{B} = C$
where:
\begin{multline*}\noindent
C = \flatmap{(k, (s_x, s_y))}{ \ite{s_y \neq \singleton{}}{\flatmap{x}{\singleton{(k,x)}}{s_x}}{\singleton{}}}{\cogroup{B}{A}}
\end{multline*}

We have: $$C =\!\!\!\!\!\! \biguplus_{(k,(s_x, s_y)) \in \cogroup{B}{A}}~~ \biguplus_{x \in s_x} (\ite{s_y \neq \singleton{}}{\singleton{(k,(x,y))}}{\singleton{}})$$

(1) Let $e \in C$.
So $\exists (k,(s_x, s_y))) \in \cogroup{B}{A}$ such that $\exists x\in s_x \quad e = (k,x)$ and $s_y \neq \singleton{}$.

We have $(k,(s_x, s_y)) \in \cogroup{B}{A}$, so $s_x = \setcomp{v}{(k,v) \in B}$, which means that $(k,x) \in B$ because $x \in s_x$.
And $s_y \neq \singleton{}$ means that $\exists w \; (k,w) \in A$,
so $e = (k,x) \in \semijoinfilter{B}$.


(2) Let $(k,x) \in \semijoinfilter{B}$.
We have $(k,x) \in B$ and $\exists w \; (k,w) \in A$.
So $k \in \opname{keys}(A) \sunion \opname{keys}(B)$.

Let $s_x = \setcomp{v}{(k,v) \in B}$ and $s_y = \setcomp{v}{(k,y) \in A}$, so  $(k, (s_x, s_y)) \in \cogroup{B}{A}$.

Since $x \in s_x$ and  $s_y \neq \singleton{}$ (because $\exists w \; (k,w) \in A$), then $(k,x) \in C$.

